Deciphering stellar chorus: apollinaire, a Python 3 module for Bayesian peakbagging in helio- and asteroseismology

Since the asteroseismic revolution, availability of efficient and reliable methods to extract stellar-oscillation mode parameters has been one of the keystone of modern stellar physics. In the helio- and asteroseismology fields, these methods are usually referred as peakbagging. We introduce in this paper the apollinaire module, a new Python 3 open-source Markov Chains Monte Carlo (MCMC) framework dedicated to peakbagging. The theoretical framework necessary to understand MCMC peakbagging methods for disk-integrated helio- and asteroseismic observations are extensively described. In particular, we present the models that are used to estimate the posterior probability function in a peakbagging framework. A description of the apollinaire module is then provided. We explain how the module enables stellar background, p-mode global pattern and individual-mode parameters extraction. By taking into account instrumental specificities, stellar inclination angle, rotational splittings, and asymmetries, the module allows fitting a large variety of p-mode models suited for solar as well as stellar data analysis with different instruments. After having been validated through a Monte Carlo fitting trial on synthetic data, the module is benchmarked by comparing its outputs with results obtained with other peakbagging codes. An analysis of the PSD of 89 one-year subseries of GOLF observations is performed. Six stars are also selected from the Kepler LEGACY sample in order to demonstrate the code abilities on asteroseismic data. The parameters we extract with apollinaire are in good agreement with those presented in the literature and demonstrate the precision and reliability of the module.

==> golf_example.tex <==
\section{Example of extraction of solar p-mode parameters in GOLF data with the \peakbagging function \label{appendix:golf_peakbagging}}

This section presents the result of a fit performed on helioseismic data with the \peakbagging function. The considered time series is a one year series obtained with GOLF (from 29/06/1996 to 29/06/1997).
The fit has been performed on the $n=20$ even pair with splittings, asymmetries and $l=4,5$ leaks taken into account. The MCMC was sampled with 500 walkers and 1000 iterations. The 100 first iterations have been discarded. 
The corner plot summarising the fit in Fig.~\ref{fig:example_golf_20_02} has been directly produced by the \texttt{peakbagging} function. Each parameter of the $l=2$ mode has been set to vary freely with no constraint from the $l=0$ modes parameters.  The correlation between mode heights and widths can be observed in the 2D marginalised distributions.

\begin{figure*}
    \centering
    \includegraphics[width=1.\textwidth]{figures/mcmc_sampler_order_20_degrees_02.png}
    \caption{Corner plot visualisation of the MCMC sampled with a one year GOLF series (from 29/06/1996 to 29/06/1997) for modes $M_{19,2}$ and $M_{20,0}$. The diagonal panels correspond to the 1D marginalised parameter distributions while the other panels correspond to the 2D parameter marginalised distributions.}
    \label{fig:example_golf_20_02}
\end{figure*}
